Combinatorial Identities for Vacillating Tableaux

Vacillating tableaux are sequences of integer partitions that satisfy specific conditions. The concept of vacillating tableaux stems from the representation theory of the partition algebra and the combinatorial theory of crossings and nestings of matchings and set partitions. In this paper, we further investigate the enumeration of vacillating tableaux and derive multiple combinatorial identities and integer sequences relating to the number of vacillating tableaux, simplified vacillating tableaux, and limiting vacillating tableaux.

==> References.tex <==

% Keyword: Initial + last two digit 

\begin{thebibliography}{99}


\bibitem{BH17} G. Benkart, T. Halverson. 
Partition Algebras and the Invariant Theory of the Symmetric Group. 
in Recent Trend in Combinatorics, 
ed:  H\'{e}l\`{e}ne Barcelo, Gizem Karaali, Rosa Orellana. 
Association for Women in Mathematics Series, volume 16. 2019. 
arXiv:1709.07751


\bibitem{BHPYZ} Z.~Berikkyzy,  P.~E.~Harris, A.~Pun, C.~Yan, and C.~Zhao. 
On the limiting vacillating tableaux for integer sequences. 
\emph{Journal of Combinaotorics}.  2023. 

\bibitem{BHH17} 
G.~Benkart, T.~Halverson, and N.~Harman, Dimensions of irreducible modules for partition algebras and tensor power multiplicities for symmetric and alternating groups, 
\emph{J.
Algebr. Combin}. 46 no. 1 (2017), 77-108; arXiv:1605.06543.

\bibitem{CDDSY07} 
W.~Y.~C.~Chen, E.~Y.~P.~Deng, R.~R.~X.~Du, R.~P.~Stanley and C.~H.~ Yan.
{Crossings and nestings of matchings and set partitions }.  
\emph{Trans. Amer. Math. Soc}. volume 359, no. 4, (2007) 1555--1575.
 


\bibitem{COSSZ} L.~Colmenarejo, R.~Orellana,  F.~Saliola, A.~Schilling, and M.~Zabrocki. An insertion algorithm of multiset partitions with applications to diagram algebras. 
\emph{Journal of Algebra}, 
557, 1(2020),  97-128. arXiv:1905.02071v2. 



\bibitem{GP11} 
A.~M.~Goyt and L.~K.~Pudwell. Solution to Monthly  problem 11567. May, 2011. 
 https://faculty.valpo.edu/lpudwell/papers/MonthlyStirling.pdf

\bibitem{GuoP20}
 Ting Guo and Svetlana Poznanovi ́c. Hecke insertion and maximal increasing and de- creasing sequences in fillings of stack polyominoes. 
 \emph{J. Combina. Theory, Series A}, 
 176:105304, 11, 2020.
 
\bibitem{HJ18} T.~Halverson and T.~N.~Jacobson. 
Set-partition tableaux and representations of diagram algebras. 
 \emph{Algebraic Combinatorics}, Volume 3 (2020) no. 2, 509-538.
arXiv:1808.08118. 




\bibitem{HL05} T.~Halverson and  T.~Lewandowski. 
RSK insertion for set partitions and diagram algebras.
\emph{Electron J. Combin.} 11 (2004/2006), 24. 


\bibitem{HR13} T.~Halverson and M.~Reeks.~Gelfand Models for Diagram Algebras. 
\emph{Journal of Algebraic Combinatorics: An International Journal}, 
Volume 41, Issue 2, March 2015.  229–255. 

\bibitem{HT10} T.~Halverson and N.~Thiem. 
$q$-Partition algebra combinatorics. 
\emph{J. Cocmbin. Theory A}, 117(2010), 507--527. 

\bibitem{Knuth70} D.E.~Knuth. Permutations, Matrices, and Generalized Young Tbleaux. 
\emph{Pacific J.  Math.}  34 No.3(1970), 709-- 727. 

\bibitem{Kratten06} C.~Krattenthaler. 
Growth diagrams, and increasing and decreasing chains in fillings of Ferrrers shapes. 
\emph{Adv. Appl. Math.} 37(2006), 404--431. 

\bibitem{Kratten23} C.~Krattenthaler. 
Identities for vacillating tableaux via growth diagrams. 
\href{https://arxiv.org/abs/2304.07657}{ArXiv:2304.07657}. 


\bibitem{MR98} P.P.~Martin and G.~Rollet, The Potts model representation and a Robinson–Schensted correspondence
for the partition algebra, \emph{Compositio Math}. 112 (1998), 237–254.

\bibitem{NM15} S.~Nkonkobe, V.~Murali. A study of a family of generating functions of Nelsen-Schmidt type and some identities on restricted barred preferential arrangements. 
arXiv: 1503.06172. 

\bibitem{OZ15} R.~Orellana and M.~Zabrocki, Symmetric group characters as symmetric functions,
arXiv:1605.06672v2. 

\bibitem{Robinson38} 
G. de B. Robinson, On the Representations of the Symmetric Group, 
\emph{Amer. J. Math}. 60 (1938), no. 3, 745–760. \MR{1507943}

\bibitem{Rubey11} 
M. Rubey.  Increasing and decreasing sequences in fillings of moon polyominoes, \emph{Adv. in Appl.
Math.} 47 (2011),  57–87.

\bibitem{OEIS} N.~J.~A.~Sloane. The On-line Encyclopedia of Integer Sequences. \href{https://oeis.org/}{https://oeis.org}.  

\bibitem{Sagan01} B.~Sagan. the Symmetric Groups, Representations, Combinatorial Algorithms, and Symmetric Functions, second edition, Springer-Verlag, New York, 2001. 


\bibitem{EC2} R.~Stanley. Enumerative Combinatorics, Vol. 2, Cambridge University Press, Cambridge, 1999. 


\bibitem{Sch61} C.~Schensted, Longest increasing and decreasing subsequences. \emph{Canad. J. Math.} 13 (1961), 179--191. \MR{0121305} 

\bibitem{Sunderam90} 
S. Sundaram, The Cauchy identity for Sp(2n), J. Combin. Theory Ser. A, 53 (1990), 209–238.

\end{thebibliography}


